Evolution of Optimization Algorithms for Global Placement via Large Language Models

Optimization algorithms are widely employed to tackle complex problems, but designing them manually is often labor-intensive and requires significant expertise. Global placement is a fundamental step in electronic design automation (EDA). While analytical approaches represent the state-of-the-art (SOTA) in global placement, their core optimization algorithms remain heavily dependent on heuristics and customized components, such as initialization strategies, preconditioning methods, and line search techniques. This paper presents an automated framework that leverages large language models (LLM) to evolve optimization algorithms for global placement. We first generate diverse candidate algorithms using LLM through carefully crafted prompts. Then we introduce an LLM-based genetic flow to evolve selected candidate algorithms. The discovered optimization algorithms exhibit substantial performance improvements across many benchmarks. Specifically, Our design-case-specific discovered algorithms achieve average HPWL improvements of \textbf{5.05\%}, \text{5.29\%} and \textbf{8.30\%} on MMS, ISPD2005 and ISPD2019 benchmarks, and up to \textbf{17\%} improvements on individual cases. Additionally, the discovered algorithms demonstrate good generalization ability and are complementary to existing parameter-tuning methods.

==> Makefile <==
ENGINE := pdflatex --shell-escape
BIB := bibtex

PROJECT := main

all:
	$(ENGINE) $(PROJECT).tex
	$(BIB)    $(PROJECT)
	$(BIB)    $(PROJECT)
	$(ENGINE) $(PROJECT).tex
	$(ENGINE) $(PROJECT).tex

fast:
	$(ENGINE) $(PROJECT).tex

clean:
	rm *.log *.aux *.blg *.bbl *.gz *.dvi *.thm *.dat *.out *latexmk *fls *busy\)


==> doc/cover.tex <==
{
%\twocolumn[
%\begin{@twocolumnfalse}
%\large

\noindent Dear Editor and Reviewers,

\ \\
Thank you very much for reviewing and editing our submission.
Enclosed is our manuscript entitled \textit{``
    Evolution of Optimization Algorithms for Global Placement via Large Language Models
''}.
This is an original paper that has not been published anywhere else.
We look forward to contributing to IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems (TCAD).
Thank you in advance for your efforts on reviewing and editing.

\ \\
Best regards,

\ \\

\noindent 
Xufeng Yao

%\end{@twocolumnfalse}
%]
}


==> pdfplot/runtime-ai/Makefile <==
ENGINE := pdflatex
BIB := bibtex

PROJECT := runtime-ai

all:
	$(ENGINE) $(PROJECT).tex
	$(BIB)    $(PROJECT)
	$(BIB)    $(PROJECT)
	$(ENGINE) $(PROJECT).tex
	$(ENGINE) $(PROJECT).tex

fast:
	$(ENGINE) $(PROJECT).tex


clean:
	rm -f *.log *.aux *.blg *.bbl *.gz *.dvi \
		*.thm *.dat *.out *.run.xml *.bcf *.data


==> pdfplot/runtime-autodmp/Makefile <==
ENGINE := pdflatex
BIB := bibtex

PROJECT := run-time

all:
	$(ENGINE) $(PROJECT).tex
	$(BIB)    $(PROJECT)
	$(BIB)    $(PROJECT)
	$(ENGINE) $(PROJECT).tex
	$(ENGINE) $(PROJECT).tex

fast:
	$(ENGINE) $(PROJECT).tex


clean:
	rm -f *.log *.aux *.blg *.bbl *.gz *.dvi \
		*.thm *.dat *.out *.run.xml *.bcf *.data

